Neuron Patching: Semantic-based Neuron-level Language Model Repair for Code Generation

Language Models (LMs) have become widely used in software engineering, especially for tasks such as code generation, where they are referred to as code LMs. These models have proven effective in generating code, making it easier for developers to automate coding activities. However, research has highlighted a significant limitation: despite their effectiveness, LMs often produce code that is incorrect, buggy, or not fully functional. Updating these models with limited data can be prohibitively challenging, yet it is essential to maximize their utility. This may require hot-fix techniques (updating models with limited data) to resolve. In this paper, we propose \ul{M}odel \ul{I}mprovement via \ul{N}euron \ul{T}argeting (\textsc{MINT}), a novel approach for repairing code LMs. MINT leverages the semantic property of language models to perform neuron-level repairs in a novel way. Further, by analyzing the relationships between the model's latent representations, the incorrect outputs, and the desired outputs, \textsc{MINT} determines which neurons are worth updating. This approach ensures that only the neurons crucial to the model's failure are targeted, avoiding unnecessary changes and allowing for a more efficient and precise repair process. \textsc{MINT} is effective, efficient, and reliable, capable of correcting a neural model by patching a minimum number of neurons (usually one or two neurons). Our approach is evaluated on three coding tasks: line-level code generation, shellcode generation, and intent-to-bash translation. The experimental results demonstrate that the proposed approach significantly outperforms the state-of-the-art in both effectiveness and efficiency measures. In addition, we analyze and discuss the side effects of model repair techniques, including the balance between generalization and specificity, and the performance after multiple repairs in succession.

==> front/ccs.tex <==
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002944.10011122.10002945</concept_id>
<concept_desc>General and reference~Surveys and overviews</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010257.10010293.10010294</concept_id>
<concept_desc>Computing methodologies~Neural networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011006.10011041.10011047</concept_id>
<concept_desc>Software and its engineering~Source code generation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{General and reference~Surveys and overviews}
\ccsdesc[500]{Computing methodologies~Neural networks}
\ccsdesc[500]{Software and its engineering~Source code generation}

==> front/copyright.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{XXXXXXX.XXXXXXX}


%%
%% These commands are for a JOURNAL article.
\acmJournal{JACM}
\acmVolume{37}
\acmNumber{4}
\acmArticle{111}
\acmMonth{8}

%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% For managing citations, it is recommended to use bibliography
%% files in BibTeX format.
%%
%% You can then either use BibTeX with the ACM-Reference-Format style,
%% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
%% support for advanced citation of software artefact from the
%% biblatex-software package, also separately available on CTAN.
%%
%% Look at the sample-*-biblatex.tex files for templates showcasing
%% the biblatex styles.
%%

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

==> listings/ladder.tex <==
\begin{algorithm}
% \SetAlgoLined
\SetKwData{Idx}{idx}
\KwData{array $A$ having $n$ elements; target element $A[t]$}
\KwResult{array $A$ where the target element swapped itself with smallest larger elements in turn}

\Repeat{$\Idx < 0$}{
    \Idx $\leftarrow$ $-1$\;
    \For{$i \leftarrow 0$ \KwTo $n-1$}{
        \If{$A[i] > A[t]$}{
            \If{$\Idx < 0$ \textbf{or} $A[i] < A[\Idx]$}{
                \Idx $\leftarrow$ $i$\;
            }
        }
    }
    \tcp{swap both values and places}
    $A[t]$, $A[\Idx]$ $\leftarrow$ $A[\Idx]$, $A[t]$\;
    $t$ $\leftarrow$ \Idx\;
}
\caption{Virtual Distribution Construction.}
\label{algo:ladder}
\end{algorithm}


==> listings/lerp.tex <==
\begin{lstlisting}[language=Python,label={lst:lerp},caption=Linear Interpolation in Python]
def interpolate_tractions(num_layers: int, inputs_rep: Tensor, outputs_rep: Tensor) => dict[int, Tensor]:
    """"compute tractions using linear interpolation"""
    layer_tractions = {0: inputs_rep}
    for layer_idx in range(num_layers):
        context_rep = torch.lerp(inputs_rep, outputs_rep, (layer_idx + 1) / num_layers)
        layer_tractions[layer_idx] = context_rep
    return layer_tractions
\end{lstlisting}

==> sections/3.benchmark.tex <==
\section{Benchmark}
\label{sec:benchmark}

To avoid the costly and biased study of the generalization ability on massive data, we build a benchmark to quantify generalization and specificity. It can also detect under-fitting and over-fitting issues in model repair.

\subsection{Problem Setting}

Model repair can solve an LM failure by patching a few neurons. We want to examine that model repair has a proper generalization ability, namely a solve model failure can affect more than one datum, as long as the data is related.

\paragraph{\textbf{Generalization}}
Generalization is the trait that the changes in a certain knowledge are insensitive to wording and context.

We prepare related data that has the same ground truth to predict as the next token.
If a specific LM failure undergoes model repair that elevates the target token to its argmax token, it is expected that the related data, which shares the common ground truth for the next-token prediction, will also have the target token closer to or even become the argmax token.

\paragraph{\textbf{Specificity}}
Specificity refers to the degree of targeted knowledge changes that do not affect other knowledge.

We prepare irrelevant data that has different tokens as the ground truth to predict the next token.
If a specific LM failure undergoes model repair that elevates the target token to its argmax token, it is \emph{not} expected that irrelevant data, which has a different ground truth for next-token prediction, will have the target token closer to or even become the argmax token.

% the side effects on other top tokens, since their targets are different, should be minimized. This ensures that the evaluation of all these target tokens becomes more reliable.

As the criterion, we measure the changes happening in both the ranking and probability of target tokens for both generalization and specificity.
For the former, we focus on the changes in the relevant data, while for the latter, in the irrelevant data.
% For the former, we focus on the relevant data (the same next-token for predictions) while for the latter, we focus on the irrelevant data (different next-tokens for predictions).
Even though the changes of other non-target tokens are also worth attention, especially the top tokens, their changes may not be as obvious as the target token.

% \paragraph{\textbf{Capacity}}
% Capacity means the maximum number of editing actions before the performance of a certain aspect is affected.

% For the study on capacity, there is no need to specify different target tokens in data preparation, nor collect similar data for each datum. The model editing will be conducted in a general way.

% We propose a novel measure to study the capacity of model editing named ``Neuron Fatigue''. Inspired by the process of ``metal fatigue'', which refers to the weakening or damage that occurs in a metal structure over time due to repeated strain.
% For each token to edit, after the normal edit-action is completed, we still repeat the edit-action (keep selecting the token at a specific ranking as the target token), and the edit-action will gradually become different and even worse in its effects.
% We trace the generated top tokens after each edit action until there appear changes on the top tokens, which indicates the edit neuron becomes fatigued, and the side effects have been unignorable.
% We use the maximum number of harmless editing cycles ($2$ edit-actions per cycle) as the criterion.

\subsection{Manual-crafted Process}

The benchmark has a total data size of $450$. As shown in \cref{tab:benchmark}, it covers $3$ types and $15$ subtypes. In each subtype, there are $30$ data samples, that is $10$ crafted samples times by $3$ generated variants.

\paragraph{\textbf{Data Type and Subtypes}}
To represent general features in Python programs, we want the LM failures can cover the diverse properties, including operators, keywords, and API names of different functionalities, to guarantee the sample diversity. Therefore, we include $3$ types and $15$ subtypes in the benchmark.

\paragraph{\textbf{Token Pairs}}
In each subtype of the benchmark, we prepare $3$ pairs of argmax tokens and target tokens. The argmax token is fixed, so for each argmax token, we prepare $3$ varied target tokens for good universality.

\paragraph{\textbf{Data Samples}}
For each pair of tokens, we manually craft $10$ different data samples that contain the argmax tokens, and they can cover the common usages of corresponding properties, to increase the data scale of the benchmark.

\begin{table}[!tb]
    \caption{Statistics of the Benchmark}
    \label{tab:benchmark}
    \centering
    \resizebox{1.0\linewidth}{!}{
        \input{tables/bench.glance}
    }
\end{table}

\subsection{Usage}
\label{subsec:benchmark:usage}

When doing next-token prediction, we start at the position to predict the argmax token, since every data sample contains the specified argmax token. We want to obtain the target token as the argmax token so will carry out model repair there.
% However, in some cases where the designed argmax token is not the actual argmax token, it is needed to do one additional edit-action before we do the evaluation.

We iterate the benchmark and let each datum be the \textit{patch set} to do model repair, and dynamically collect the relevant data and irrelevant data from the benchmark as the \textit{probe sets}. The size of the patch set is $1$, and we have two probe sets collocated with each patch set, separately for generation and specificity.
The datum from the probe sets will do next-token prediction before and after model repair.

In the benchmark, for a datum to undergo model repair, we collect the data of the same subtype as the probe set for generalization study, noted as $G$. Since they have the same argmax token, they tend to share the same knowledge, they will need the same target token to be the new argmax token.
In contrast, we collect the data of different subtypes as the probe set for specificity study, noted as $S$. The reason is that, the data having no common argmax token are hard to express the same knowledge, so they won't need the current target token to be the new argmax token.
We limit the scope to the same type of data, so the specificity study can be more strict. We repeat the computation on three types of data and check their average performance.

In addition, we can evaluate the changes in rankings and probabilities of the target token to quantify generalization and specificity.
A large change means good generalization on $G$ since the effect of model repair on relevant data is positive, but it means bad specificity on $S$ since the effect of model repair on irrelevant data is negative.

Let's take an example, assuming a datum belonging to the ``assign'' subtype is the patch set for model repair, we take the other data in the ``assign'' subtype as the probe set $G$ for generalization, containing $9$ elements; and collect the data from the ``assign\_multiply'', ``arithmetic\_mod'', ``logic\_and'', ``comparison\_ge'' subtypes as the probe set $S$ for specificity, containing $40$ elements.
When the target token ``\verb|+|'' is the argmax token in model repair, we expect the same effects on other data of the ``assign'' subtype, but we won't expect that to affect the data of other subtypes.
For the same subtype, the performance in other cases will also be studied, where the target token is ``\verb|%|'' or ``\verb|~|''.
Similarly, the computation will repeat on all $450$ data samples.
The scores on different data types will be averaged as an overall measure of the generalization and the specificity.

% For the study on capacity, the designed target tokens will not be used.


==> sections/9.application.tex <==
\section{Application: LM Reasoning}

Based on the capability of model repair on correcting generative LMs, it can further guide LM reasoning.
The former disturbs the priorities of predicted tokens; while the latter alters specific knowledge in reasoning.
We give two examples to show its effects.

In our examples, ``$\Rightarrow$'' and ``$\rightarrow$'' indicate direct and indirect changes, and underlined tokens are the points where a change may happen.
For each underlined token to predict, the prompt is its recent chain-of-thought contents in italics appended with its prefixed tokens.

% That is, once we correct a factual truth in the model, other knowledge stored in the model, especially these relevant neurons could benefit from the editing actions.

% As discussed above, the neuron-level model repair pipeline is composed of several steps, therefore the whole performance is dependent on the quality of its core components.
% For example, an excessively greedy heuristic objective might cause an ``overfitting'' issue in a generation, that is, the edited target token might still be ranked at high places in following generations.
% Similarly, mild heuristic traction will improve the editing process, such as reducing the required number of editing, and further, reduce potential side effects to the model.

% \input{listings/lerp}

% , we connect it with the corresponding code generation using a chain of thought, as shown below:

\begin{custombox}
    [`print' in Python2 is a statement, then print the constant `PI':print PI\\
    `print' in Python3 is a function, then print the constant `PI':print(PI)]
    \\\textbf{Patch: }
    `assert' in Python3 is a\uline{ statement}$\Rightarrow$\uline{ function}
    \\\textbf{Probe: }
    `assert' in Python2 is a\uline{ statement}, assert that the variable `age' is larger than 0:assert\uline{ age>0}
    \\\textbf{Probe: }
    `assert' in Python3 is a\uline{ statement}$\rightarrow$\uline{ function}, assert that the variable `age' is larger than 0:assert\uline{ age > 0}$\rightarrow$\uline{(age > 0)}
\end{custombox}

First, we demonstrate that LM's behavior directly dependent on a patched knowledge will change accordingly, let's say, the usage of a Python keyword changed.
For the factual knowledge in Code LM that ```assert' in Python3 is a statement'', we inject a counterfactual by model repair, that is, making the model believe `assert' in Python3 is a function instead of a statement.
As shown below, the model turns to believe `assert' in Python3 is indeed a function, no longer a statement, but it still believes `assert' in Python2 is a statement.
Further, when the model writes an assertion in Python3, it uses the syntax of a function, no longer a statement, but it still uses the syntax of a statement in Python2.

% After an edit action, the rankings of tokens ``function'' and ``statement'' get switched.
% Therefore, the model automatically switches to another chain-of-thought, and then the code LM can successively output ``assert(PI>0)'' instead of ``assert PI>0'' for the given query. The changed chain-of-thought is as shown below:

\begin{custombox}
    [the SciPy API to compute Cosine distance is `distance.cosine()'\\
    the SciPy API to compute Euclidean distance is `distance.euclidean()']
    \\\textbf{Patch: }
    the SciPy API to compute Manhattan distance is `distance.
    \uline{manhattan()}$\Rightarrow$\uline{cityblock()}'
    \\\textbf{Probe: }
    the SciPy API to compute Chebyshev distance is `distance.
    \uline{chebyshev()}'
    \\\textbf{Probe: }
    the SciPy API to compute Manhattan distance is `distance.
    \uline{manhattan()}$\rightarrow$\uline{cityblock()}'
    \\\textit{the crane workload can be estimated using the Chebyshev distance}
    \\\textit{the forklift workload can be estimated using the Manhattan distance}
    \\\textbf{Probe: }
    the SciPy API to estimate the crane workload is `dist = distance.\uline{cdist()}'
    \\\textbf{Probe: }
    the SciPy API to estimate the forklift workload is `dist = distance.\uline{cdist()}$\rightarrow$\uline{cityblock()}'
\end{custombox}

Then, we demonstrate that LM's behavior indirectly dependent on a patched knowledge will change accordingly as well, for example, the name of a SciPy API changed.
For the hallucination in Code LM that ``the SciPy API to compute Manhattan distance is `distance.manhattan()''', we correct it with the actual knowledge by model repair, that is, making the model accept `distance.cityblock()' is the right API to invoke.
As shown below, the model turns to understand `cityblock()' is exactly the API to compute the Manhattan distance, no longer the imagined `manhattan()'. Meanwhile, its behavior to compute the Chebyshev distance remains unchanged, still by using `chebyshev()'.
Further, when the model writes a line of code to estimate the forklift workload, it is using the oriented `cityblock()', no longer a general `cdist()'. In contrast, the model still uses `cdist()' as a common way to estimate the crane workload.
It should be mentioned that, in the second two probes, the context has changed to the contents of the connections between workloads and distances. In the real world, these chain-of-thoughts might be hidden, with no need to be explicitly given.

% In the above cases, the effects of model repair in reasoning can be well shown.
Overall, enabled by model repair, LM's behaviors can change accordingly for patched knowledge, no matter whether their dependencies are direct or indirect.
For this reason, model repair is more ideal than rule-based methods which require additional processing.

% It is the sequence caused by our one-time editing operation even though the initial purpose is merely editing knowledge.

% Our model repair could fulfill both scenes. However, there are still limitations to overcome for wider applications.

% \subsection{Threats to Validity}
%%% also append our attempts to reduce threats

% \paragraph{\textbf{Internal Validity}}
% Our model repair approach \textsc{MINT} is strongly supported by the experiments and measures. Also, our work mainly cares about the basic aspect of leveraging neural models for generative tasks, that is, matrix operations and probability computation. Therefore, our findings are credible and reliable.

% \paragraph{\textbf{External Validity}}
% In our understanding, our model repair approach \textsc{MINT} can smoothly generalize to different Transformer models, and meanwhile, guarantee its effectiveness. 
% Our experiments cover different data and tasks, so our model can generalize to more data and tasks.
% However, it may be challenging to significantly improve neural models when their basic capability is weak, that is, model repair cannot play the role of model finetuning.


==> tables/experiment.baseline.tex <==
\sisetup{table-format=2.2}
\begin{tabular}{
    l cc ccc cc
}

\toprule

\multirow{2}[2]{*}{\textbf{Approach}} & \multicolumn{2}{c}{\textbf{Prerequisite}} & \multicolumn{2}{c}{\textbf{Granularity}} & \multicolumn{3}{c}{\textbf{Applicability}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
& {\textbf{Trigger Tokens}} & {\textbf{Parallel Data}}
& {\textbf{Layer Level}} & {\textbf{Neuron Level}}
& {\textbf{Encoder-only}} & {\textbf{Decoder-only}} & {\textbf{Encoder-Decoder}} \\

\midrule

\textsc{ROME}~\cite{Meng2022LocatingAE}
& \xmark & \-
& \cmark & \-
& \- & \cmark & \- \\
\textsc{MEMIT}~\cite{Meng2022MassEditingMI}
& \xmark & \-
& \cmark & \-
& \- & \cmark & \- \\
\textsc{KN}~\cite{Dai2021KnowledgeNI}
& \- & \xmark
& \- & \cmark
& \cmark & \cmark & \cmark \\

\midrule

\textsc{MINT} (Ours)
& \- & \-
& \- & \cmark
& \cmark & \cmark & \cmark \\

\bottomrule

\end{tabular}


==> tables/results.rq4.capacity.tex <==
\sisetup{table-format=2.2}
\begin{tabular}{
    l rrrr rrrr rrrr
}

\toprule

\multirow{2}[2]{*}{\textbf{Approach}} & \multicolumn{4}{c}{\textbf{FR (\#0$\leftrightarrows$\#1) YieldRate}} & \multicolumn{4}{c}{\textbf{FR (\#0$\leftrightarrows$\#2) YieldRate}} & \multicolumn{4}{c}{\textbf{FR (\#0$\leftrightarrows$\#3) YieldRate}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& {\textbf{0.5$\uparrow$}} & {\textbf{0.667$\uparrow$}} & {\textbf{0.75$\uparrow$}} & {\textbf{0.8$\uparrow$}}
& {\textbf{0.5$\uparrow$}} & {\textbf{0.667$\uparrow$}} & {\textbf{0.75$\uparrow$}} & {\textbf{0.8$\uparrow$}}
& {\textbf{0.5$\uparrow$}} & {\textbf{0.667$\uparrow$}} & {\textbf{0.75$\uparrow$}} & {\textbf{0.8$\uparrow$}} \\

\midrule

\expttag{\textsc{MINT} [std.]}
& 0.978 & 0.889 & 0.889 & 0.733
& 0.111 & 0.022 & 0.022 & 0.022
& 0.0 & 0.0 & 0.0 & 0.0 \\
% \cline{3-4}\cline{7-9}

\midrule

\expttag{[loc.-1-actv]}
& \tabh 0.978 & \tabh 0.889 & \tabh 0.889 & \tabh 0.822
& 0.089 & \tabh 0.067 & \tabh 0.044 & \tabh 0.022
& \tabh 0.044 & 0.0 & 0.0 & 0.0 \\
% \cline{3-4}

\expttag{[loc.-1-rand]}
& 0.467 & 0.378 & 0.289 & 0.222
& \tabh \text{0.267} & \tabh 0.022 & 0.0 & 0.0
& \tabh 0.333 & \tabh 0.044 & \tabh 0.022 & \tabh 0.022 \\
% \cline{12-13}

\midrule

\expttag{[est.-1-pathway]}
& 0.711 & 0.711 & 0.711 & 0.711
& \tabh 0.111 & \tabh 0.067 & \tabh 0.044 & \tabh 0.022
& \tabh 0.044 & \tabh 0.022 & \tabh 0.022 & \tabh 0.022 \\
% \cline{2-5}\cline{11-13}

\midrule

\expttag{[est.-2-onehot]}
& \tabh 0.978 & \tabh \text{0.978} & \tabh \text{0.978} & \tabh \text{0.933}
& 0.067 & 0.0 & 0.0 & 0.0
& 0.0 & 0.0 & 0.0 & 0.0 \\

\expttag{[est.-2-switch]}
& 0.6 & 0.444 & 0.378 & 0.156
& 0.022 & 0.0 & 0.0 & 0.0
& 0.0 & 0.0 & 0.0 & 0.0 \\
% \cline{2-4}

\midrule

\expttag{[plan-1-score]}
& 0.733 & 0.489 & 0.289 & 0.222
& \tabh 0.178 & \tabh 0.067 & \tabh 0.022 & \tabh 0.022
& 0.0 & 0.0 & 0.0 & 0.0 \\
% \cline{8-9}

\midrule

\expttag{[plan-2-steady]}
& 0.289 & 0.244 & 0.244 & 0.2
& \tabh \text{0.267} & \tabh \text{0.267} & \tabh \text{0.267} & \tabh \text{0.267}
& \tabh \text{0.356} & \tabh \text{0.333} & \tabh \text{0.333} & \tabh \text{0.333} \\
% \cline{3-4}\cline{6-9}\cline{11-13}

\midrule

\expttag{[plan-3-prob]}
& 0.933 & 0.778 & 0.733 & 0.667
& \tabh 0.111 & \tabh 0.044 & \tabh 0.044 & \tabh 0.044
& \tabh 0.022 & 0.0 & 0.0 & 0.0 \\
% \cline{7-9}

\expttag{[plan-3-rank]}
& \tabh 0.978 & 0.622 & 0.378 & 0.244
& \tabh 0.156 & 0.0 & 0.0 & 0.0
& 0.0 & 0.0 & 0.0 & 0.0 \\

\bottomrule

\end{tabular}
